WebGLM: Towards An Efficient Web-Enhanced Question Answering System with Human Preferences

We present WebGLM, a web-enhanced question-answering system based on the General Language Model (GLM). Its goal is to augment a pre-trained large language model (LLM) with web search and retrieval capabilities while being efficient for real-world deployments. To achieve this, we develop WebGLM with strategies for the LLM-augmented retriever, bootstrapped generator, and human preference-aware scorer. Specifically, we identify and address the limitations of WebGPT (OpenAI), through which WebGLM is enabled with accuracy, efficiency, and cost-effectiveness advantages. In addition, we propose systematic criteria for evaluating web-enhanced QA systems. We conduct multi-dimensional human evaluation and quantitative ablation studies, which suggest the outperformance of the proposed WebGLM designs over existing systems. WebGLM with the 10-billion-parameter GLM (10B) is shown to perform better than the similar-sized WebGPT (13B) and even comparably to WebGPT (175B) in human evaluation. The code, demo, and data are at \url{https://github.com/THUDM/WebGLM}.

==> sections/4_dataset.tex <==
\section{Dataset}

In order to help training models for answering in a long form to the questions with references materials, we introduced \textbf{WebRefQA}, a dataset consisting of \textbf{Q}uestion-\textbf{A}nswer pairs with \textbf{Ref}erences from \textbf{Web}sites. The main procedure of this dataset are shown in Fig. \ref{fig:web_ref_qa}

\begin{figure}[ht]
    \includegraphics[width=\linewidth]{figures/web_ref_qa.png}
    \caption{\textbf{WebRefQA}.} 
    \label{fig:web_ref_qa}
\end{figure}

\begin{figure}[ht]
    \includegraphics[width=\linewidth]{figures/prompt.jpg}
    \caption{The prompt method in data collection process we finally adopt. First list several references indexed by a number with brackets, then state the question and provide a prompt word "Answer". \textcolor{blue}{Blue} parts are prompts.} 
    \label{fig:prompt}
\end{figure}

\begin{figure*}[ht]
    \includegraphics[width=\textwidth]{figures/instruction_induction.jpg}
    \caption{figure caption}
    \label{fig:instruction-induction}
\end{figure*}

\begin{figure*}[ht]
    \includegraphics[width=\textwidth]{figures/in-context.jpg}
    \caption{figure caption}
    \Description{figure description}
    \label{fig:in-context}
\end{figure*}



\subsection{Formulation}

Formally, \textbf{WebRefQA} can be formulated as a set $\mathcal{D(Q,A,R,C)}$, where:

\begin{displaymath}
\mathcal{C} \subseteq \mathcal{Q}\times\mathcal{A}\times 2^{\mathcal{R}}
\end{displaymath}

$\mathcal{Q}$, $\mathcal{A}$, $\mathcal{R}$ represents the question set, the answer set and the reference set respectively. $\mathcal{C}$ represents the relations among the three sets defined above.

Each element $\alpha\in \mathcal{A}$ can be represented as

[This following part is redundant to 3.methodology]

\begin{displaymath}
\alpha = (<s_1, r_1>, <s_2, r_2>, \cdots, <s_n, r_n>)
\end{displaymath}

$<s_k, r_k>$ represents the \textit{k-th} segment in answer $\alpha$, where $s_k$ is a text sequence and $r_k\subset \mathcal{R}$ is a subset of references, indicating $s_k$ refers to $r_k$.

In terms of data organization, each example in \textbf{WebRefQA} contains four fields:
\begin{itemize}
    \item {\verb|Question|}: The question from ELI5 \cite{eli5}.
    \item {\verb|References|}: References collected by searching via Google API, fetching original pages, extracting plain text, scoring paragraphs and picking the high score ones.
    \item {\verb|URLs|}: The website links of corresponding references.
    \item {\verb|Answer|}: The answer produced by GPT-3 \cite{gpt3} with instruction-guided in-context learning methods.
\end{itemize}

\subsection{Data Collection}

In order to enable the model to learn the ability to distinguish all references provided and pick related ones, our references should not be over-filtered, but should retain well-related ones and noise at the same time. Our search methods are designed to satisfy this need.

The work of Unnatural Instructions \cite{Unnatural_Instructions} demonstrated that model-generated data could be an effective alternative in terms of both cost and performance. The experiments on GPT-3 have indicated that in-context learning can achieve strong performance on many NLP tasks\cite{gpt3}. 

Generally, the approaches to collecting data can be described as follow steps.

\subsubsection{Prompt Selecting}

 We compare several types of prompts, including the orders between question and its corresponding references, the symbols used to mark the indices of references, and the prompt words of references and questions. We conduct experiments with every type of prompt we have mentioned, and finally find a natural way as shown in Fig.\ref{fig:prompt} performs best. 


\subsubsection{Instruction Inducting}

Instruction induction \cite{instruction_induction} inspires us that not only can human design instructions to conduct in-context learning, but large language models can also generate instructions by giving a few examples. Fig.\ref{fig:instruction-induction}  shows our instruction generating prompting.

\subsubsection{In-Context Generation}

One-shot learning and few-shot learning have both been experimented on GPT-3\cite{gpt3}, results of two methods share similar performance. One-shot learning can even sometimes surpass few-shot learning in terms of answer's quality if the total length of references is too large. We finally conduct generation by one-shot learning as shown in Fig.\ref{fig:in-context}, and over 80,000 data have been collected.


\subsubsection{Filtering}

The original data generated by model can not be applied to training process because of the hallucination of model and citation mistake in generating. We design a method to filter these data. We will discard a piece of data if it satisfies any condition below: 1) There are only few citations in answer; 2) Any of citation indices is invalid, such as noting a nonexistent reference index; 3) The accuracy of citation is too low. We make decision that whether a reference should be cited by a text segment via 1-gram overlap. This threshold is the one which performs best on WebGPT \cite{webgpt} examples.

\subsubsection{Citation Recomposing}

We split each answer into segments by their corresponding citations and compute reference matching score for each segment in order to build ideal citations. Finally, we compose text sequences and corresponding ideal citations into a new answer.

After these steps, the final training dataset contains about 26,000 triplets of question, answer and corresponding references.


\subsection{Data Version: Filter methods}

Note: This can be an Ablation Study.

We conduct experiments on datasets with various filter methods. 

In the first version of our dataset, we implement no filter methods after retrieval. We surprisingly find that the performance of an answer to a question closely related to its citation accuracy. So as a result, we filter our dataset on citation accuracy. In the second version of our dataset, we implement a Rouge-L[] method on citation. And in the third version, we implement a 1-gram method instead.

We explain two vital things in this section. One is how we design our filters, and how to select a threshold whether to regard a citation positive or negative. The other is why we select 1-gram instead of Rouge-L method.

\subsubsection{Filter Design} For in-context generation, GPT-3 model can learn the latent citation position, but it may incorrectly cite an irrelevant reference. So we split the generated answer into segments by citation marks. Then we calculate the precision score of each pair of answer segments and all references. We pick a threshold, we regard positive citation if the score are not less than the threshold. Otherwise, a citation should be regard as a negative one. Finally, we calculate F-measure of all the citations.

WebGPT [] shows its 272 examples. We try each threshold on it, and find that when we use Rouge-L, the best threshold is 0.4, and the best one is 0.57 when we use Rouge-1. 

[Algorithm or formulation statement can be inserted here.]

\subsubsection{Why 1-gram} We find a fact that large language models are able to compose a reference into a new sentence, and sometimes they exchange the order of some phrases. In this situation, an answer may hold a low Rouge-L score but a high Rouge-1 score.

